A Practical Method for Generating String Counterfactuals

Interventions targeting the representation space of language models (LMs) have emerged as an effective means to influence model behavior. Such methods are employed, for example, to eliminate or alter the encoding of demographic information such as gender within the model's representations and, in so doing, create a counterfactual representation. However, because the intervention operates within the representation space, understanding precisely what aspects of the text it modifies poses a challenge. In this paper, we give a method to convert representation counterfactuals into string counterfactuals. We demonstrate that this approach enables us to analyze the linguistic alterations corresponding to a given representation space intervention and to interpret the features utilized to encode a specific concept. Moreover, the resulting counterfactuals can be used to mitigate bias in classification through data augmentation.

==> diagram.tex <==


\begin{figure*}[t]
\centering
\usetikzlibrary{arrows.meta, calc, positioning, shapes, matrix}

% Colors
\definecolor{femaleColor}{HTML}{FBB13C}   % Light orange
\definecolor{maleColor}{HTML}{6CB4EE}     % Light blue
\definecolor{nnColor}{HTML}{A5D6A7}       % Light green
\definecolor{conceptColor}{HTML}{8E44AD}  % Purple for concept emphasis
\definecolor{boxLine}{HTML}{333333}       % Dark line color

\begin{tikzpicture}[
  font=\footnotesize,
  node distance=0.4cm,
  >=Stealth,
  every node/.style={align=left}
]

% Box styles
\tikzset{
  boxText/.style={
    rectangle,
    rounded corners=2pt,
    draw=boxLine,
    thick,
    text width=2.8cm,  % Narrower boxes
    inner sep=3pt,
    font=\footnotesize
  },
  repBox/.style={
    rectangle,
    rounded corners=2pt,
    draw=boxLine,
    thick,
    minimum width=1.6cm,
    minimum height=0.7cm,
    font=\footnotesize,
    align=center
  },
  conceptLabel/.style={
    text=conceptColor,
    font=\bfseries
  }
}

% Matrix arrangement: 2 rows, 3 columns
\matrix[column sep=1.6cm, row sep=0.8cm] (m) {
  % -------------------- Top row --------------------
  \node[boxText, fill=femaleColor!15, text width=4cm] (origText) {
    \textbf{C = (Female)}\\[2pt]
  {\small
    She received \underline{her} undergraduate degree from Emory University
    and \underline{her} J.D.\ from the University of Houston Law Center.
    Jacqueline and \underline{her} husband, Ian,
    enjoy raising their three children.
  }
  }; &
  \node[boxText, fill=nnColor!25] (encoder) {
    \textbf{Encoder}\\{\scriptsize Neural Network}
  }; &
  \node[repBox, fill=femaleColor!15] (xfem) {
    $\mathbf{X}_{f}$\\
    {\tiny Female}
  }; \\

  % -------------------- Bottom row --------------------
  \node[repBox, fill=maleColor!20] (xmal) {
    $\mathbf{X}_{m}$\\
    {\tiny Male}
  }; &
  \node[boxText, fill=nnColor!25] (inversion) {
    \textbf{Vec2Text}\\{\scriptsize Inversion model}
  }; &
  \node[boxText, fill=maleColor!15, text width=4cm] (cfText) {
    \textbf{C = (Male)}\\[2pt]
    {\small He received \underline{his} undergraduate degree from Houston College of Law
    and \underline{his} J.D.\ from Emory University.
    Ian and \underline{his} wife, Jacqueline, have three wonderful children.
    In \underline{his} free time, Ian enjoys spending time with \underline{his} family.}
  }; \\
};

% Arrows & Labels
% Top row arrows
\draw[->, thick] (origText.east) -- node[above, font=\scriptsize]{Encode} (encoder.west);
\draw[->, thick] (encoder.east) -- node[above, font=\scriptsize]{Representation} (xfem.west);

% Bottom row arrows
\draw[->, thick] (xfem.south) -- ++(0,-1.6) -| node[left, pos=0.25, font=\scriptsize]{} (xmal.north);
\draw[->, thick] (xmal.east) -- node[above, font=\scriptsize]{} (inversion.west);
\draw[->, thick] (inversion.east) -- node[above, font=\scriptsize]{String \\ Counterfactual} (cfText.west);

% Concept Shift Label
\node[conceptLabel, yshift=5pt] at ($(xfem)!0.5!(xmal)$) {\emph{Representation Surgery}};

\end{tikzpicture}
\caption{\footnotesize
A schematic illustration of \textbf{counterfactual lens} demonstrated for gender concept.
We first encode the original text (\textcolor{femaleColor}{female}) to obtain its vector representation $\mathbf{X}_{\textsc{f}}$. 
We apply \emph{representation surgery}, i.e, steer or erase a particular concept (e.g., gender) to produce $\mathbf{X}_{\textsc{m}}$. 
Finally, we invert the representation-level counterfactual to obtain a textual counterfactual for the alternate concept value (\textcolor{maleColor}{male}).
}
\label{fig:intervention-lens}
\end{figure*}



